Safe Reinforcement Learning with Chance-constrained Model Predictive Control

Real-world reinforcement learning (RL) problems often demand that agents behave safely by obeying a set of designed constraints. We address the challenge of safe RL by coupling a safety guide based on model predictive control (MPC) with a modified policy gradient framework in a linear setting with continuous actions. The guide enforces safe operation of the system by embedding safety requirements as chance constraints in the MPC formulation. The policy gradient training step then includes a safety penalty which trains the base policy to behave safely. We show theoretically that this penalty allows for a provably safe optimal base policy and illustrate our method with a simulated linearized quadrotor experiment.

==> di_system_fig.tex <==
\begin{tikzpicture}[declare function={
        g(\x)=2*exp(-(\x+6)*(\x+6)/2); 
        f(\x)=2*exp(-(\x-6)*(\x-6)/2); 
        gxmin=-9;gxmax=-3;
        fxmin=3;fxmax=9;}]
    
    \draw [thick] (-2,0.25) -- (4,0.25);
    \draw[red!80!black,line width = 1mm] (-2,-0.25) -- (-2,0.75);
    \draw[red!80!black,line width = 1mm] (4,-0.25) -- (4,0.75);
    \fill[black] (2,0) rectangle (2.5,0.5);
    \draw [-stealth](2.25,1) -- (3,1) node [left,xshift=-0.8cm] {$\dot x$};
    
    \path (4,0.5) node[left]{$x_{\max}$};
    \path (-1,0.5) node[left]{$x_{\min}$};

    \begin{scope}[x=3pt,y=3pt,shift={(2.25cm,-1cm)}]
      \draw[gray!50,thick] (-12,0) -- (12,0);
      \draw[gray!50,thick] (0,-5) -- (0,5);
      \draw[thick,green!60!black] plot[domain=gxmin:gxmax,samples=51,smooth] (\x,{g(\x)}) node [left,yshift=15] {$\polsafe$}; 
      \draw[thick] plot[domain=fxmin:fxmax,samples=51,smooth] (\x,{f(\x)}) node [right,yshift=15,xshift=-10] {$\pol$}; 
        \path (12,-0.25) node[right]{$u$};
    \end{scope}
\end{tikzpicture}


==> diexperiment.tex <==
\begin{figure}[tbp]
\floatconts
{fig:diexample}% label for whole figure
{\caption{Experimental setup and results for the double integrator setting. (a) The safety guide corrects an unsafe action distribution from the base policy. (b) The safety sets for the double integrator system. The dashed lines represent the true bounds of the terminal safety set $\stsafeterm$; we inner approximate this by a polytope. In practice, we also slightly shrink $x_{\min}$ and $x_{\max}$ by some factor $1-\delta$. (c) Test-time performances of a policy gradient agent trained with and without the safety guide on the double integrator task. The thick line indicates mean performance over five runs, with the shaded area representing the standard deviation.}}% caption for whole figure
{%
\subfigure[][t]{
%\vspace{-0.6cm}
\label{fig:doubleint}% label for this sub-figure
\resizebox{.28\textwidth}{!}{\input{di_system_fig}}
}
\qquad % space out the images a bit
\subfigure[][t]{%
\label{fig:disafetyset}% label for this sub-figure
\resizebox{.28\textwidth}{!}{\input{safetyset_fig}}
}
\qquad % space out the images a bit
\subfigure[][t]{
\label{fig:diresults}
\includegraphics[width=0.28\textwidth]{result.png}
}
}
\end{figure}

\label{sec:experiments}
\subsection{Double integrator}
Consider a one-dimensional point mass as depicted in Figure~\ref{fig:doubleint}. The system state vector is $\st = [x_t, \dot x_t] \T$, where $x_t$ represents the position of the mass at time step $t$. The episode terminates if the position of the mass leaves the interval $[x_{\min}, x_{\max}]$, and the reward $\re(\st, \ac) = {\dot x}_t^2$ is simply the square of the velocity at each time step. The control input $\ac \in [a_{\min}, a_{\max}]$ is the force on the point mass. Using the time step $\Delta t = 0.02$, the dynamics evolve according to
\[
    \begin{bmatrix}
        x_{t+1} \\
        \dot x_{t+1}
    \end{bmatrix} =
    \begin{bmatrix}
        1 & \Delta t \\
        0 & 1
    \end{bmatrix}
    \begin{bmatrix}
        x_t \\
        \dot x_t
    \end{bmatrix}
    +
    \begin{bmatrix}
        0 \\
        1
    \end{bmatrix}
    \ac
\]
We set $[x_{\min}, x_{\max}] = [-1, 1]$ and our safe set $\stsafe$ to be the slightly smaller $[-0.9, 0.9]$. Our terminal safe set $\stsafeterm$ consists of the same position bounds as well as a position-dependent velocity bound that represents the maximum velocity that can be brought to zero by the end of the interval. Since this curve scales with the square root of distance, we inner approximate this by a polytope---see Figure~\ref{fig:disafetyset}. The safety tolerance and planning horizon parameters are set as $\epsilon = 0.001$ and $H = 30$. The safety penalty we set at $\beta = 1.5$. Our network consists of two hidden layers of size $64$ with $\tanh$ nonlinearities. We collected $5000$ steps per batch and update with the learning rate $0.001$ and discount factor $\gamma = 0.97$. The safety guide optimization problem is solved using MOSEK \citep{mosek}.

We compare the performances of a policy gradient agent trained with and without the safety guide in Figure~\ref{fig:diresults}. The vanilla policy gradient agent learns a short-sighted policy of simply accelerating through the end of the interval and does not improve beyond a reward of $50$. However, since the safety guided policy is prevented from hitting the end of the interval, it is able to explore in the other direction and eventually discover the optimal strategy of oscillating back and forth between the two end points, yielding a much higher performance.



==> old.tex <==
\section{Electronic Submission}
\label{submission}




\subsection{Author Information for Submission}
\label{author info}

ICML uses double-blind review, so author information must not appear. If
you are using \LaTeX\/ and the \texttt{icml2021.sty} file, use
\verb+\icmlauthor{...}+ to specify authors and \verb+\icmlaffiliation{...}+ to specify affiliations. (Read the TeX code used to produce this document for an example usage.) The author information
will not be printed unless \texttt{accepted} is passed as an argument to the
style file.
Submissions that include the author information will not
be reviewed.

\subsubsection{Self-Citations}

If you are citing published papers for which you are an author, refer
to yourself in the third person. In particular, do not use phrases
that reveal your identity (e.g., ``in previous work \cite{langley00}, we
have shown \ldots'').

Do not anonymize citations in the reference section. The only exception are manuscripts that are
not yet published (e.g., under submission). If you choose to refer to
such unpublished manuscripts \cite{anonymous}, anonymized copies have
to be submitted
as Supplementary Material via CMT\@. However, keep in mind that an ICML
paper should be self contained and should contain sufficient detail
for the reviewers to evaluate the work. In particular, reviewers are
not required to look at the Supplementary Material when writing their
review.

\subsubsection{Camera-Ready Author Information}
\label{final author}

If a paper is accepted, a final camera-ready copy must be prepared.
%
For camera-ready papers, author information should start 0.3~inches below the
bottom rule surrounding the title. The authors' names should appear in 10~point
bold type, in a row, separated by white space, and centered. Author names should
not be broken across lines. Unbolded superscripted numbers, starting 1, should
be used to refer to affiliations.

Affiliations should be numbered in the order of appearance. A single footnote
block of text should be used to list all the affiliations. (Academic
affiliations should list Department, University, City, State/Region, Country.
Similarly for industrial affiliations.)

Each distinct affiliations should be listed once. If an author has multiple
affiliations, multiple superscripts should be placed after the name, separated
by thin spaces. If the authors would like to highlight equal contribution by
multiple first authors, those authors should have an asterisk placed after their
name in superscript, and the term ``\textsuperscript{*}Equal contribution"
should be placed in the footnote block ahead of the list of affiliations. A
list of corresponding authors and their emails (in the format Full Name
\textless{}email@domain.com\textgreater{}) can follow the list of affiliations.
Ideally only one or two names should be listed.

A sample file with author names is included in the ICML2021 style file
package. Turn on the \texttt{[accepted]} option to the stylefile to
see the names rendered. All of the guidelines above are implemented
by the \LaTeX\ style file.

\subsection{Abstract}

The paper abstract should begin in the left column, 0.4~inches below the final
address. The heading `Abstract' should be centered, bold, and in 11~point type.
The abstract body should use 10~point type, with a vertical spacing of
11~points, and should be indented 0.25~inches more than normal on left-hand and
right-hand margins. Insert 0.4~inches of blank space after the body. Keep your
abstract brief and self-contained, limiting it to one paragraph and roughly 4--6
sentences. Gross violations will require correction at the camera-ready phase.

\subsection{Partitioning the Text}

You should organize your paper into sections and paragraphs to help
readers place a structure on the material and understand its
contributions.

\subsubsection{Sections and Subsections}

Section headings should be numbered, flush left, and set in 11~pt bold
type with the content words capitalized. Leave 0.25~inches of space
before the heading and 0.15~inches after the heading.

Similarly, subsection headings should be numbered, flush left, and set
in 10~pt bold type with the content words capitalized. Leave
0.2~inches of space before the heading and 0.13~inches afterward.

Finally, subsubsection headings should be numbered, flush left, and
set in 10~pt small caps with the content words capitalized. Leave
0.18~inches of space before the heading and 0.1~inches after the
heading.

Please use no more than three levels of headings.

\subsubsection{Paragraphs and Footnotes}

Within each section or subsection, you should further partition the
paper into paragraphs. Do not indent the first line of a given
paragraph, but insert a blank line between succeeding ones.

You can use footnotes\footnote{Footnotes
should be complete sentences.} to provide readers with additional
information about a topic without interrupting the flow of the paper.
Indicate footnotes with a number in the text where the point is most
relevant. Place the footnote in 9~point type at the bottom of the
column in which it appears. Precede the first footnote in a column
with a horizontal rule of 0.8~inches.\footnote{Multiple footnotes can
appear in each column, in the same order as they appear in the text,
but spread them across columns and pages if possible.}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Figures}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
Figure~\ref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Algorithms}

If you are using \LaTeX, please use the ``algorithm'' and ``algorithmic''
environments to format pseudocode. These require
the corresponding stylefiles, algorithm.sty and
algorithmic.sty, which are supplied with this package.
Algorithm~\ref{alg:example} shows an example.

\begin{algorithm}[tb]
   \caption{Bubble Sort}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $x_i$, size $m$
   \REPEAT
   \STATE Initialize $noChange = true$.
   \FOR{$i=1$ {\bfseries to} $m-1$}
   \IF{$x_i > x_{i+1}$}
   \STATE Swap $x_i$ and $x_{i+1}$
   \STATE $noChange = false$
   \ENDIF
   \ENDFOR
   \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
Table~\ref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.

\subsection{Citations and References}

Please use APA reference format regardless of your formatter
or word processor. If you rely on the \LaTeX\/ bibliographic
facility, use \texttt{natbib.sty} and \texttt{icml2021.bst}
included in the style-file package to obtain this format.

Citations within the text should include the authors' last names and
year. If the authors' names are included in the sentence, place only
the year in parentheses, for example when referencing Arthur Samuel's
pioneering work \yrcite{Samuel59}. Otherwise place the entire
reference in parentheses with the authors and year separated by a
comma \cite{Samuel59}. List multiple references separated by
semicolons \cite{kearns89,Samuel59,mitchell80}. Use the `et~al.'
construct only for citations with three or more authors or after
listing all authors to a publication in an earlier reference \cite{MachineLearningI}.

Authors should cite their own work in the third person
in the initial version of their paper submitted for blind review.
Please refer to Section~\ref{author info} for detailed instructions on how to
cite your own papers.

Use an unnumbered first-level section heading for the references, and use a
hanging indent style, with the first line of the reference flush against the
left margin and subsequent lines indented by 10 points. The references at the
end of this document give examples for journal articles \cite{Samuel59},
conference publications \cite{langley00}, book chapters \cite{Newell81}, books
\cite{DudaHart2nd}, edited volumes \cite{MachineLearningI}, technical reports
\cite{mitchell80}, and dissertations \cite{kearns89}.

Alphabetize references by the surnames of the first authors, with
single author entries preceding multiple author entries. Order
references for the same authors by year of publication, with the
earliest first. Make sure that each reference includes all relevant
information (e.g., page numbers).

Please put some effort into making references complete, presentable, and
consistent. If using bibtex, please protect capital letters of names and
abbreviations in titles, for example, use \{B\}ayesian or \{L\}ipschitz
in your .bib file.

\section*{Software and Data}

If a paper is accepted, we strongly encourage the publication of software and data with the
camera-ready version of the paper whenever appropriate. This can be
done by including a URL in the camera-ready copy. However, \textbf{do not}
include URLs that reveal your institution or identity in your
submission for review. Instead, provide an anonymous URL or upload
the material as ``Supplementary Material'' into the CMT reviewing
system. Note that reviewers are not required to look at this material
when writing their review.

% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
\nocite{langley00}

